Explaining text classifiers through progressive neighborhood approximation with realistic samples

The importance of neighborhood construction in local explanation methods has been already highlighted in the literature. And several attempts have been made to improve neighborhood quality for high-dimensional data, for example, texts, by adopting generative models. Although the generators produce more realistic samples, the intuitive sampling approaches in the existing solutions leave the latent space underexplored. To overcome this problem, our work, focusing on local model-agnostic explanations for text classifiers, proposes a progressive approximation approach that refines the neighborhood of a to-be-explained decision with a careful two-stage interpolation using counterfactuals as landmarks. We explicitly specify the two properties that should be satisfied by generative models, the reconstruction ability and the locality-preserving property, to guide the selection of generators for local explanation methods. Moreover, noticing the opacity of generative models during the study, we propose another method that implements progressive neighborhood approximation with probability-based editions as an alternative to the generator-based solution. The explanation results from both methods consist of word-level and instance-level explanations benefiting from the realistic neighborhood. Through exhaustive experiments, we qualitatively and quantitatively demonstrate the effectiveness of the two proposed methods.

==> ref_raw.tex <==
% =====================================================================================
% |                                     General                                       |
% =====================================================================================

% Survey regarding ML & DL increasing trend
@article{pouyanfar2018survey,
  title={A survey on deep learning: Algorithms, techniques, and applications},
  author={Pouyanfar, Samira and Sadiq, Saad and Yan, Yilin and Tian, Haiman and Tao, Yudong and Reyes, Maria Presa and Shyu, Mei-Ling and Chen, Shu-Ching and Iyengar, Sundaraja S},
  journal={ACM Computing Surveys (CSUR)},
  volume={51},
  number={5},
  pages={1--36},
  year={2018},
  publisher={ACM New York, NY, USA}
}

% number of parameters increased exponentially
@article{bernstein2021freely,
  title={Freely scalable and reconfigurable optical hardware for deep learning},
  author={Bernstein, Liane and Sludds, Alexander and Hamerly, Ryan and Sze, Vivienne and Emer, Joel and Englund, Dirk},
  journal={Scientific reports},
  volume={11},
  number={1},
  pages={1--12},
  year={2021},
  publisher={Nature Publishing Group}
}

% concerns & regulations regarding AI ethics
@article{goodman2017european,
  title={European Union regulations on algorithmic decision-making and a “right to explanation”},
  author={Goodman, Bryce and Flaxman, Seth},
  journal={AI magazine},
  volume={38},
  number={3},
  pages={50--57},
  year={2017}
}

% XAI Survey, show growing attention on XAI
@inproceedings{danilevsky2020survey,
  title={A Survey of the State of Explainable AI for Natural Language Processing},
  author={Danilevsky, Marina and Qian, Kun and Aharonov, Ranit and Katsis, Yannis and Kawas, Ban and Sen, Prithviraj},
  booktitle={Proceedings of the 1st Conference of the Asia-Pacific Chapter of the Association for Computational Linguistics and the 10th International Joint Conference on Natural Language Processing},
  pages={447--459},
  year={2020}
}

% XAI Survey, show growing attention on XAI
@article{linardatos2020explainable,
  title={Explainable ai: A review of machine learning interpretability methods},
  author={Linardatos, Pantelis and Papastefanopoulos, Vasilis and Kotsiantis, Sotiris},
  journal={Entropy},
  volume={23},
  number={1},
  pages={18},
  year={2020},
  publisher={MDPI}
}

% For text corruption
@article{iosifidis2019sentiment,
  title={Sentiment analysis on big sparse data streams with limited labels},
  author={Iosifidis, Vasileios and Ntoutsi, Eirini},
  journal={Knowledge and Information Systems},
  pages={1--40},
  year={2019},
  publisher={Springer}
}

% TF-IDF
@book{manning2008introduction,
  title={Introduction to information retrieval},
  author={Manning, Christopher D},
  year={2008},
  publisher={Syngress Publishing}
}

% n-gram, a book about computational linguistics in general
@book{jurafsky2000speech,
  title={Speech \& language processing},
  author={Jurafsky, Dan},
  year={2000},
  publisher={Pearson Education India}
}

% About extrinsic features 
@article{ma2017salient,
  title={Salient Region Detection by Integrating Intrinsic and Extrinsic Cues without Prior Information.},
  author={Ma, Ji and Li, Jingjiao and Li, Zhenni and Jiao, Jiao},
  journal={Journal of Engineering Science \& Technology Review},
  volume={10},
  number={3},
  year={2017}
}

% About extrinsic features 
@inproceedings{wang2011image,
  title={Image saliency: From intrinsic to extrinsic context},
  author={Wang, Meng and Konrad, Janusz and Ishwar, Prakash and Jing, Kevin and Rowley, Henry},
  booktitle={CVPR 2011},
  pages={417--424},
  year={2011},
  organization={IEEE}
}

% Diversity measure used for factual sampling
@article{gong2019diversity,
  title={Diversity in machine learning},
  author={Gong, Zhiqiang and Zhong, Ping and Hu, Weidong},
  journal={IEEE Access},
  volume={7},
  pages={64323--64350},
  year={2019},
  publisher={IEEE}
}

% LSTM
@article{hochreiter1997long,
  title={Long short-term memory},
  author={Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
  journal={Neural computation},
  volume={9},
  number={8},
  pages={1735--1780},
  year={1997},
  publisher={MIT Press}
}

% --> Talks about XAI potential usages, including debugging
@inproceedings{bhatt2020explainable,
  title={Explainable machine learning in deployment},
  author={Bhatt, Umang and Xiang, Alice and Sharma, Shubham and Weller, Adrian and Taly, Ankur and Jia, Yunhan and Ghosh, Joydeep and Puri, Ruchir and Moura, Jos{\'e} MF and Eckersley, Peter},
  booktitle={Proceedings of the 2020 conference on fairness, accountability, and transparency},
  pages={648--657},
  year={2020}
}

% debiasing 
@inproceedings{kennedy2020contextualizing,
  title={Contextualizing Hate Speech Classifiers with Post-hoc Explanation},
  author={Kennedy, Brendan and Jin, Xisen and Davani, Aida Mostafazadeh and Dehghani, Morteza and Ren, Xiang},
  booktitle={Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
  pages={5435--5442},
  year={2020}
}

% debiasing -- PoE
@inproceedings{cai2022power,
  title={Power of Explanations: Towards automatic debiasing in hate speech detection},
  author={Cai, Yi and Zimek, Arthur and Wunder, Gerhard and Ntoutsi, Eirini},
  booktitle={2022 IEEE 9th International Conference on Data Science and Advanced Analytics (DSAA)},
  pages={1--10},
  year={2022},
  organization={IEEE}
}


% =====================================================================================
% |                              For numerical data                                   |
% =====================================================================================
% TBD: merge
@inproceedings{plumb2018model,
  title={Model agnostic supervised local explanations},
  author={Plumb, Gregory and Molitor, Denali and Talwalkar, Ameet},
  booktitle={Proceedings of the 32nd International Conference on Neural Information Processing Systems},
  pages={2520--2529},
  year={2018}
}

% LIME
@inproceedings{ribeiro2016should,
  title={" Why should i trust you?" Explaining the predictions of any classifier},
  author={Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  booktitle={Proceedings of the 22nd ACM SIGKDD international conference on knowledge discovery and data mining},
  pages={1135--1144},
  year={2016}
}

% --> Theoretical study on LIME
@inproceedings{garreau2020explaining,
  title={Explaining the explainer: A first theoretical analysis of LIME},
  author={Garreau, Damien and Luxburg, Ulrike},
  booktitle={International Conference on Artificial Intelligence and Statistics},
  pages={1287--1296},
  year={2020},
  organization={PMLR}
}

% ALIME
@inproceedings{shankaranarayana2019alime,
  title={ALIME: Autoencoder based approach for local interpretability},
  author={Shankaranarayana, Sharath M and Runje, Davor},
  booktitle={International conference on intelligent data engineering and automated learning},
  pages={454--463},
  year={2019},
  organization={Springer}
}

% ANCHOR
@inproceedings{ribeiro2018anchors,
  title={Anchors: High-precision model-agnostic explanations},
  author={Ribeiro, Marco Tulio and Singh, Sameer and Guestrin, Carlos},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={32},
  number={1},
  year={2018}
}

% SHAP
@article{lundberg2017unified,
  title={A Unified Approach to Interpreting Model Predictions},
  author={Lundberg, Scott M and Lee, Su-In},
  journal={Advances in Neural Information Processing Systems},
  volume={30},
  pages={4765--4774},
  year={2017}
}

% --> Global SHAP
@article{lundberg2020local,
  title={From local explanations to global understanding with explainable AI for trees},
  author={Lundberg, Scott M and Erion, Gabriel and Chen, Hugh and DeGrave, Alex and Prutkin, Jordan M and Nair, Bala and Katz, Ronit and Himmelfarb, Jonathan and Bansal, Nisha and Lee, Su-In},
  journal={Nature machine intelligence},
  volume={2},
  number={1},
  pages={56--67},
  year={2020},
  publisher={Nature Publishing Group}
}

% Regarding perturbations
@article{vstrumbelj2009explaining,
  title={Explaining instance classifications with interactions of subsets of feature values},
  author={{\v{S}}trumbelj, Erik and Kononenko, Igor and {\v{S}}ikonja, M Robnik},
  journal={Data \& Knowledge Engineering},
  volume={68},
  number={10},
  pages={886--904},
  year={2009},
  publisher={Elsevier}
}

% Regarding perturbations, mentioned the previous one
@article{strumbelj2010efficient,
  title={An efficient explanation of individual classifications using game theory},
  author={Strumbelj, Erik and Kononenko, Igor},
  journal={The Journal of Machine Learning Research},
  volume={11},
  pages={1--18},
  year={2010},
  publisher={JMLR. org}
}

% Reference for feature independence assumption
@article{vstrumbelj2014explaining,
  title={Explaining prediction models and individual predictions with feature contributions},
  author={{\v{S}}trumbelj, Erik and Kononenko, Igor},
  journal={Knowledge and information systems},
  volume={41},
  number={3},
  pages={647--665},
  year={2014},
  publisher={Springer}
}

% LORE, genetic algorithm for neighborhood generation
@article{guidotti2018local,
  title={Local rule-based explanations of black box decision systems},
  author={Guidotti, Riccardo and Monreale, Anna and Ruggieri, Salvatore and Pedreschi, Dino and Turini, Franco and Giannotti, Fosca},
  journal={arXiv preprint arXiv:1805.10820},
  year={2018}
}

% =====================================================================================
% |                                For image data                                     |
% =====================================================================================
% TBD: merge, model-agnostic explanation for images, strategical sampling
@inproceedings{petsiuk2018rise,
  title={Rise: Randomized input sampling for explanation of black-box models},
  author={Petsiuk, Vitali and Das, Abir and Saenko, Kate},
  booktitle={British Machine Vision Conference},
  year={2018}
}

% --> GRAD-CAM family
@inproceedings{selvaraju2017grad,
  title={Grad-cam: Visual explanations from deep networks via gradient-based localization},
  author={Selvaraju, Ramprasaath R and Cogswell, Michael and Das, Abhishek and Vedantam, Ramakrishna and Parikh, Devi and Batra, Dhruv},
  booktitle={Proceedings of the IEEE international conference on computer vision},
  pages={618--626},
  year={2017}
}

% --> GRAD-CAM family
@inproceedings{chattopadhay2018grad,
  title={Grad-cam++: Generalized gradient-based visual explanations for deep convolutional networks},
  author={Chattopadhay, Aditya and Sarkar, Anirban and Howlader, Prantik and Balasubramanian, Vineeth N},
  booktitle={2018 IEEE Winter Conference on Applications of Computer Vision (WACV)},
  pages={839--847},
  year={2018},
  organization={IEEE}
}

% --> Global, self-explaining networks, knowing particular function forms
@article{puri2021cofrnets,
  title={CoFrNets: interpretable neural architecture inspired by continued fractions},
  author={Puri, Isha and Dhurandhar, Amit and Pedapati, Tejaswini and Shanmugam, Karthikeyan and Wei, Dennis and Varshney, Kush R},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={21668--21680},
  year={2021}
}

% --> an overview of LRP family
@article{montavon2019layer,
  title={Layer-wise relevance propagation: an overview},
  author={Montavon, Gr{\'e}goire and Binder, Alexander and Lapuschkin, Sebastian and Samek, Wojciech and M{\"u}ller, Klaus-Robert},
  journal={Explainable AI: interpreting, explaining and visualizing deep learning},
  pages={193--209},
  year={2019},
  publisher={Springer}
}

% LRP original
@article{bach2015pixel,
  title={On pixel-wise explanations for non-linear classifier decisions by layer-wise relevance propagation},
  author={Bach, Sebastian and Binder, Alexander and Montavon, Gr{\'e}goire and Klauschen, Frederick and M{\"u}ller, Klaus-Robert and Samek, Wojciech},
  journal={PloS one},
  volume={10},
  number={7},
  pages={e0130140},
  year={2015},
  publisher={Public Library of Science San Francisco, CA USA}
}

% LRP for RNN
@article{arras2017explaining,
  title={Explaining Recurrent Neural Network Predictions in Sentiment Analysis},
  author={Arras, Leila and Montavon, Gr{\'e}goire and M{\"u}ller, Klaus-Robert and Samek, Wojciech},
  journal={EMNLP 2017},
  pages={159},
  year={2017}
}

% LRP for Transformers
@inproceedings{ali2022xai,
  title={XAI for transformers: better explanations through conservative propagation},
  author={Ali, Ameen and Schnake, Thomas and Eberle, Oliver and Montavon, Gr{\'e}goire and M{\"u}ller, Klaus-Robert and Wolf, Lior},
  booktitle={International conference on machine learning},
  pages={435--451},
  year={2022},
  organization={PMLR}
}

% DTD
@article{montavon2017explaining,
  title={Explaining nonlinear classification decisions with deep taylor decomposition},
  author={Montavon, Gr{\'e}goire and Lapuschkin, Sebastian and Binder, Alexander and Samek, Wojciech and M{\"u}ller, Klaus-Robert},
  journal={Pattern recognition},
  volume={65},
  pages={211--222},
  year={2017},
  publisher={Elsevier}
}

% --> DeepLIFT
@inproceedings{shrikumar2017learning,
  title={Learning important features through propagating activation differences},
  author={Shrikumar, Avanti and Greenside, Peyton and Kundaje, Anshul},
  booktitle={International conference on machine learning},
  pages={3145--3153},
  year={2017},
  organization={PMLR}
}

% ABELE: Generator-based image classifier explainer
@inproceedings{guidotti2019black,
  title={Black box explanation by learning image exemplars in the latent feature space},
  author={Guidotti, Riccardo and Monreale, Anna and Matwin, Stan and Pedreschi, Dino},
  booktitle={Joint European Conference on Machine Learning and Knowledge Discovery in Databases},
  pages={189--205},
  year={2019},
  organization={Springer}
}

% =====================================================================================
% |                                For text data                                      |
% =====================================================================================
% XSPELLS
@inproceedings{lampridis2020explaining,
  title={Explaining Sentiment Classification with Synthetic Exemplars and Counter-Exemplars},
  author={Lampridis, Orestis and Guidotti, Riccardo and Ruggieri, Salvatore},
  booktitle={International Conference on Discovery Science},
  pages={357--373},
  year={2020},
  organization={Springer}
}

% XPROAX
@inproceedings{cai2021xproax,
  title={XPROAX-Local explanations for text classification with progressive neighborhood approximation},
  author={Cai, Yi and Zimek, Arthur and Ntoutsi, Eirini},
  booktitle={2021 IEEE 8th International Conference on Data Science and Advanced Analytics (DSAA)},
  pages={1--10},
  year={2021},
  organization={IEEE}
}

% =====================================================================================
% |                     Discussion on Neighborhood & Locality                         |
% =====================================================================================
% Locality based sample, the one with half-moon example --> probably could be used as example for attack
@inproceedings{laugel2018defining,
  title={Defining Locality for Surrogates in Post-hoc Interpretablity},
  author={Laugel, Thibault and Renard, Xavier and Lesot, Marie-Jeanne and Marsala, Christophe and Detyniecki, Marcin},
  booktitle={Workshop on Human Interpretability in Machine Learning (WHI)-International Conference on Machine Learning (ICML)},
  year={2018}
}

% --> discussing on-manifold neighborhood construction & potential risks in SHAP
@inproceedings{chen2020true,
  title={True to the Model or True to the Data?},
  author={Chen, Hugh and Janizek, Joseph D and Lundberg, Scott and Lee, Su-In},
  booktitle={Workshop on Human Interpretability in Machine Learning (WHI)-International Conference on Machine Learning (ICML)},
  year={2020}
}

% --> discussing necessarity of on-manifold neighborhood construction
@article{ghalebikesabi2021locality,
  title={On locality of local explanation models},
  author={Ghalebikesabi, Sahra and Ter-Minassian, Lucile and DiazOrdaz, Karla and Holmes, Chris C},
  journal={Advances in Neural Information Processing Systems},
  volume={34},
  pages={18395--18407},
  year={2021}
}

% --> off-manifold neighborhood is unrepresentative
% also use a generative model for distribution estimation (generation)
@inproceedings{frye2020shapley,
  title={Shapley explainability on the data manifold},
  author={Frye, Christopher and de Mijolla, Damien and Begley, Tom and Cowton, Laurence and Stanley, Megan and Feige, Ilya},
  booktitle={International Conference on Learning Representations},
  year={2020}
}

% reference for locality constraint
@incollection{robnik2018perturbation,
  title={Perturbation-based explanations of prediction models},
  author={Robnik-{\v{S}}ikonja, Marko and Bohanec, Marko},
  booktitle={Human and machine learning},
  pages={159--175},
  year={2018},
  publisher={Springer}
}

% =====================================================================================
% |                                 Generative model                                  |
% =====================================================================================
% VAE
@inproceedings{bowman2016generating,
  title={Generating Sentences from a Continuous Space},
  author={Bowman, Samuel and Vilnis, Luke and Vinyals, Oriol and Dai, Andrew and Jozefowicz, Rafal and Bengio, Samy},
  booktitle={Proceedings of The 20th SIGNLL Conference on Computational Natural Language Learning},
  pages={10--21},
  year={2016}
}

% DAAE
@inproceedings{shen2020educating,
  title={Educating text autoencoders: Latent representation guidance via denoising},
  author={Shen, Tianxiao and Mueller, Jonas and Barzilay, Regina and Jaakkola, Tommi},
  booktitle={International Conference on Machine Learning},
  pages={8719--8729},
  year={2020},
  organization={PMLR}
}

% AAE
@inproceedings{makhzani2015adversarial,
  title={Adversarial autoencoders},
  author={Makhzani, Alireza and Shlens, Jonathon and Jaitly, Navdeep and Goodfellow, Ian and Frey, Brendan},
  booktitle={International Conference on Learning Representations},
  year={2016}
}

% Talked about reconstruction and latent geometry problem in VAE
@inproceedings{zhao2018adversarially,
  title={Adversarially regularized autoencoders},
  author={Zhao, Junbo and Kim, Yoon and Zhang, Kelly and Rush, Alexander and LeCun, Yann},
  booktitle={International conference on machine learning},
  pages={5902--5911},
  year={2018},
  organization={PMLR}
}

% Reconstruction problem of VAE
@article{song2019latent,
  title={Latent space expanded variational autoencoder for sentence generation},
  author={Song, Tianbao and Sun, Jingbo and Chen, Bo and Peng, Weiming and Song, Jihua},
  journal={IEEE Access},
  volume={7},
  pages={144618--144627},
  year={2019},
  publisher={IEEE}
}

% Reconstruction problem of VAE
@inproceedings{dai2020usual,
  title={The usual suspects? Reassessing blame for VAE posterior collapse},
  author={Dai, Bin and Wang, Ziyu and Wipf, David},
  booktitle={International Conference on Machine Learning},
  pages={2313--2322},
  year={2020},
  organization={PMLR}
}

% Bias in generators
@inproceedings{huang2020reducing,
  title={Reducing Sentiment Bias in Language Models via Counterfactual Evaluation},
  author={Huang, Po-Sen and Zhang, Huan and Jiang, Ray and Stanforth, Robert and Welbl, Johannes and Rae, Jack and Maini, Vishal and Yogatama, Dani and Kohli, Pushmeet},
  booktitle={Findings of the Association for Computational Linguistics: EMNLP 2020},
  pages={65--83},
  year={2020}
}

% Bias in generators
@inproceedings{sheng2021societal,
  title={Societal Biases in Language Generation: Progress and Challenges},
  author={Sheng, Emily and Chang, Kai-Wei and Natarajan, Prem and Peng, Nanyun},
  booktitle={Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
  pages={4275--4293},
  year={2021}
}

% Bias in generators
@inproceedings{amini2019uncovering,
  title={Uncovering and mitigating algorithmic bias through learned latent structure},
  author={Amini, Alexander and Soleimany, Ava P and Schwarting, Wilko and Bhatia, Sangeeta N and Rus, Daniela},
  booktitle={Proceedings of the 2019 AAAI/ACM Conference on AI, Ethics, and Society},
  pages={289--295},
  year={2019}
}

% =====================================================================================
% |                                     Dataset                                       |
% =====================================================================================
% Yelp
@inproceedings{shen2017style,
  title={Style transfer from non-parallel text by cross-alignment},
  author={Shen, Tianxiao and Lei, Tao and Barzilay, Regina and Jaakkola, Tommi},
  booktitle={Proceedings of the 31st International Conference on Neural Information Processing Systems},
  pages={6833--6844},
  year={2017}
}

% Amazon
@inproceedings{zhang2015character,
  title={Character-level convolutional networks for text classification},
  author={Zhang, Xiang and Zhao, Junbo and LeCun, Yann},
  booktitle={Proceedings of the 28th International Conference on Neural Information Processing Systems-Volume 1},
  pages={649--657},
  year={2015}
}

% amazon Review, origin
@inproceedings{mcauley2013hidden,
  title={Hidden factors and hidden topics: understanding rating dimensions with review text},
  author={McAuley, Julian and Leskovec, Jure},
  booktitle={Proceedings of the 7th ACM conference on Recommender systems},
  pages={165--172},
  year={2013}
}

% =====================================================================================
% |                                  XAI Evaluation                                   |
% =====================================================================================
% Human-grounded evaluation
@article{carvalho2019machine,
  title={Machine learning interpretability: A survey on methods and metrics},
  author={Carvalho, Diogo V and Pereira, Eduardo M and Cardoso, Jaime S},
  journal={Electronics},
  volume={8},
  number={8},
  pages={832},
  year={2019},
  publisher={Multidisciplinary Digital Publishing Institute}
}

% 3 Cs
@incollection{silva2018towards,
  title={Towards complementary explanations using deep neural networks},
  author={Silva, Wilson and Fernandes, Kelwin and Cardoso, Maria J and Cardoso, Jaime S},
  booktitle={Understanding and Interpreting Machine Learning in Medical Image Computing Applications},
  pages={133--140},
  year={2018},
  publisher={Springer}
}

% 3 Cs
@article{nauta2022anecdotal,
  title={From anecdotal evidence to quantitative evaluation methods: A systematic review on evaluating explainable ai},
  author={Nauta, Meike and Trienes, Jan and Pathak, Shreyasi and Nguyen, Elisa and Peters, Michelle and Schmitt, Yasmin and Schl{\"o}tterer, J{\"o}rg and van Keulen, Maurice and Seifert, Christin},
  journal={arXiv preprint arXiv:2201.08164},
  year={2022}
}

% A survey on XAI involving fidelity
@article{guidotti2018survey,
  title={A survey of methods for explaining black box models},
  author={Guidotti, Riccardo and Monreale, Anna and Ruggieri, Salvatore and Turini, Franco and Giannotti, Fosca and Pedreschi, Dino},
  journal={ACM computing surveys (CSUR)},
  volume={51},
  number={5},
  pages={1--42},
  year={2018},
  publisher={ACM New York, NY, USA}
}

% Explanation-guided manipulation
@inproceedings{lertvittayakumjorn2019human,
  title={Human-grounded Evaluations of Explanation Methods for Text Classification},
  author={Lertvittayakumjorn, Piyawat and Toni, Francesca},
  booktitle={Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)},
  pages={5198--5208},
  year={2019}
}

% --> TBD: also about texts, should enrich the related work, Explanation-guided manipulation
@inproceedings{arras2016explaining,
  title={Explaining Predictions of Non-Linear Classifiers in NLP},
  author={Arras, Leila and Horn, Franziska and Montavon, Gr{\'e}goire and M{\"u}ller, Klaus-Robert and Samek, Wojciech},
  booktitle={Proceedings of the 1st Workshop on Representation Learning for NLP},
  pages={1--7},
  year={2016}
}

% AOPC
@article{samek2016evaluating,
  title={Evaluating the visualization of what a deep neural network has learned},
  author={Samek, Wojciech and Binder, Alexander and Montavon, Gr{\'e}goire and Lapuschkin, Sebastian and M{\"u}ller, Klaus-Robert},
  journal={IEEE transactions on neural networks and learning systems},
  volume={28},
  number={11},
  pages={2660--2673},
  year={2016},
  publisher={IEEE}
}

% Text augmentation guiding stability evaluation
@inproceedings{rudinger2018gender,
  title={Gender Bias in Coreference Resolution},
  author={Rudinger, Rachel and Naradowsky, Jason and Leonard, Brian and Van Durme, Benjamin},
  booktitle={Proceedings of NAACL-HLT},
  pages={8--14},
  year={2018}
}

% Text augmentation guiding stability evaluation
@inproceedings{dixon2018measuring,
  title={Measuring and mitigating unintended bias in text classification},
  author={Dixon, Lucas and Li, John and Sorensen, Jeffrey and Thain, Nithum and Vasserman, Lucy},
  booktitle={Proceedings of the 2018 AAAI/ACM Conference on AI, Ethics, and Society},
  pages={67--73},
  year={2018}
}
